Two Dimensional Conformal Field Theory and a Primer to Chiral Algebras

We review various aspects of two dimensional conformal field theories paying close attention to the algebraic structures that intervene. We provide a compact description regarding the appearance of a chiral algebra as the symmetry algebra related to local conformal symmetry, namely the Virasoro algebra. We then introduce two dimensional conformal field theories with additional symmetries in which extended chiral algebras emerge as a natural generalization of the conformal case.

==> ConformalFieldtheory.tex <==
In this section we will review some of the main aspects of conformal field theory, we will use thoroughly throughout this text. We will start by introducing the conformal group in $d$ dimensions and the corresponding Lie algebra: this will be extended to it's supersymmetric counterpart in the next section. We will then focus on conformal field theories in two dimensions and conclude by introducing the notion of chiral algebras. Standard references in this topic are \cite{Francesco, Ginsparg}.  Some conceptual and fixing ideas were also taken from \cite{tong,eberhardt}.

\subsection{Conformal Symmetry in $d>2$}

\subsubsection{The Conformal Group in $d>2$ Dimensions}
\label{sec:conformalgroup}

We consider the space $\mathbb{R}^d$ with flat metric $\eta_{\mu \nu}$ of signature $(p,q)$. Under a change of coordinates $x \mapsto x'$, we have 
\begin{equation}
    \eta_{\mu \nu}\mapsto \eta'_{\mu \nu}=\frac{\partial x^\rho}{\partial x'^{\mu}}\frac{\partial x^{\sigma}}{\partial x'^{\nu}}\eta_{\rho \sigma}\,.
\end{equation}
The conformal group is defined as the group of coordinate transformations that leaves the metric invariant up to a scale change, 
\begin{equation}
\label{ec:conformalcondition}
    \eta_{\mu \nu}'=\Omega^2(x)\eta_{\mu \nu}\,.
\end{equation}
The coordinate transformations that satisfy this property, for $d>2$ are the following:

\begin{enumerate}
    \item Lorentz transformations, 
    \begin{equation}
        x^\mu \mapsto x'^{\mu}=\Lambda^{\mu}{}_\nu x^\nu \,.
    \end{equation}
    Indeed, Lorentz transformations preserve the metric, and thus $\Omega^2(x)=1$. 
    \item Translations, 
    \begin{equation}
        x^\mu \mapsto x'^\mu=x^\mu + a^\mu
    \end{equation}
    for constant $a^\mu$. A translation is again an isometry and thus $\Omega^2(x)=1$. 
    \item Dilations, 
    \begin{equation}
        x \mapsto x'= Dx 
    \end{equation}
    where $D \in \mathbb{R}$. In this case $\Omega^2(x)=D^2$.
    \item Special conformal transformations,
    \begin{equation}
     x^\mu \mapsto x'^\mu = \frac{x^\mu + |x|^2 K^\mu }{1 + 2 x^\nu K_\nu + |x|^2|K|^2}
    \end{equation}
    for constant $K^\mu$. Special conformal transformations can be constructed as the composition of $\text{inversion}\circ \text{translation}\circ \text{inversion}$, and the scale factor is given by $\Omega^2(x)=(1 + 2 x^\nu K_\nu + |x|^2|K|^2)^{-2}$.
\end{enumerate}
The set of all possible transformations of this kind form the conformal group, which is ismorphic to $SO(p+1,q+1)$. 

\subsubsection{The Conformal Algebra in $d>2$ Dimensions}

The associated Lie algebra to the conformal group, is naturally isomorphic to $\frak{so}(p+1,q+1)$ and is generated by the Lorentz generators $M^{\mu \nu}$, the generator of translations $P^\mu$, the generator of dilations $D$ and the generator of special conformal transformations $K^\mu$. These satisfy the commutation relations:
\begin{equation}
    \begin{array}{c}
         [M^{\mu \nu}, M^{\rho \sigma}]=\eta^{\nu \rho}M^{\mu \sigma} + \eta^{\mu \sigma}M^{\nu \rho}-\eta^{\mu \rho}M^{\nu \sigma}-\eta^{\nu \sigma}M^{\mu \rho} \,, \\
        & [M^{\mu \nu},P^\sigma]=\eta^{\nu \sigma}P^\mu - \eta^{\mu \sigma}P^\nu \,, \\
        &
          [M^{\mu \nu},K^\sigma]=\eta^{\nu \sigma}K^\mu - \eta^{\mu \sigma}K^\nu \,, \\
          &
         [D,P^\mu]=P^\mu\,, \\
         &
         [D,K^\mu]=-K^\mu\,, \\
         &
        [K^\mu,P^\nu]=2\left(\eta^{\mu \nu}D-M^{\mu \nu}\right)\,, 
    \end{array}
\end{equation}
where unspecified commutators vanish. In section \ref{sec:supersymetry} we will extend the Conformal Algebra in $d=4$ dimensions to its supersymmetric counterpart. 

\subsection{Conformal Symmetry in $d=2$}

In the previous subsections we introduced both the conformal group and the conformal algebra in $d>2$. Here we will talk about conformal symmetry in 2 dimensions which requires special attention. We will see that the whole group theoretic structure in the two dimensional case can be understood from a completely different perspective using the power of complex analysis. This will provide a profound insight which will enable us to understand the emergence of infinite dimensional symmetry groups and its far reaching consequences. 

\subsubsection{Global Conformal Transformations}

To make contact with the previous section, we start by defining the \textit{global conformal group} in two dimensions. Following section \ref{sec:conformalgroup}, we have that the global conformal group is the group consisting of globally defined, invertible and finite conformal transformation and is given by $SO(2,2)\cong SL(2,\mathbb{C})/\mathbb{Z}_2$. The Lie algebra associated to the global conformal group is therefore $\frak{sl}(2,\mathbb{C})\cong \frak{sl}(2,\mathbb{R})\times \overline{\frak{sl}(2,\mathbb{R})}$. Concretely, we may define two sets of generators in terms of the conformal generators as:

\begin{equation}
    \begin{array}{c}
         L_{+1}=\frac{1}{2}(K^1-iK^2)\,, \quad \quad \bar{L}_{+1} =\frac{1}{2}(K^1+iK^2) \\
         \\
         L_{0}=\frac{1}{2}(D-iM_{12})\,, \quad \quad \bar{L}_{0} =\frac{1}{2}(D+iM_{12}) \\
         \\
         L_{+1}=\frac{1}{2}(P^1+iP^2)\,, \quad \quad \bar{L}_{+1} =\frac{1}{2}(P^1-iP^2) \\
    \end{array}
\end{equation}
which separately satisfy the usual $\frak{sl}(2,\mathbb{R})$ commutation relations:

\begin{equation}
    \begin{array}{c}
         [L_{+1},L_{-1}]=2L_0\,, \quad [L_0,L_{\pm 1}]=\mp L _{\pm 1} \\
         & [\bar{L}_{+1},\bar{L}_{-1}]=2\bar{L}_0\,, \quad [\bar{L}_0,\bar{L}_{\pm 1}]=\mp \bar{L}_{\pm 1} \,.
    \end{array}
\end{equation}
We thus observe that the \textit{global} conformal algebra, which is the Lie algebra associated to the global conformal group can be expressed as two copies of the finite dimensional Lie algebra $\frak{sl}(2,\mathbb{R})$. 

\subsubsection{Local Conformal Transformations}

Things get really interesting when we relax the condition of \textit{globally} defined transformations. In order to do this, let us consider coordinates $(x^0,x^1)$ in the plane. Under a coordinate transformation, the conformal condition given in equation \eqref{ec:conformalcondition}, is equivalent to a set of Cauchy Riemmann equations for complex coordinates $z$ and $\bar{z}$ defined in terms of $x^0$ and $x^1$ as:
\begin{equation}
    z=x^{0}+i x^{1}\,, \quad \bar{z}=x^{0}-i x^{1} \,.
\end{equation}
This implies, that \textit{locally}, any analytic transformation of the complex coordinates $z$ and $\bar{z}$ will be conformal.

If we want to study the associated Lie algebra, we consider an infinitesimal transformation of the complex coordinates:
\begin{equation}
    z \mapsto z'=z+\epsilon (z)\,,\quad \bar{z}\mapsto \bar{z}'=\bar{z}+\bar{\epsilon}(\bar{z})\,.
\end{equation}
The only requirement for these transformations to be conformal is that $\epsilon(z)$ and $\bar{\epsilon}(\bar{z})$ are holomorphic and anti holomorphic functions of $z$ and $\bar{z}$ respectively in some open set $U\subseteq \mathbb{C}$. More generally, we may assume that $\epsilon(z)$ is a meromorphic function, with isolated singularities outside $U$. Hence, both $\epsilon(z)$ and $\bar{\epsilon}(\bar{z})$ admit a well defined Laurent expansion:
\begin{equation}
\label{ec:epsilonexpansion}
\begin{array}{c}
z^{\prime}=z+\epsilon(z)=z+\displaystyle\sum_{n \in \mathbb{Z}} \epsilon_{n} z^{n+1}, \\ \\
\bar{z}^{\prime}=\bar{z}+\bar{\epsilon}(\bar{z})=\bar{z}+\displaystyle\sum_{n \in \mathbb{Z}} \bar{\epsilon}_{n}\bar{z}^{n+1},
\end{array}
\end{equation}
where the infinitesimal parameters $\epsilon_n$ and $\bar{\epsilon}_n$ are constant. The effect of such a mapping on a spinless and dimensionless field defined in the plane $\phi(z,\bar{z})$ is:
\begin{equation}
\begin{split}
    \phi(z',\bar{z}')
    &=\phi(z,\bar{z})-\epsilon(z)\partial\phi(z,\bar{z})-\bar{\epsilon}(\bar{z})\bar{\partial}\phi(z,\bar{z})\\
    &=\phi(z,\bar{z})+\sum_{n \in \mathbb{Z}}\epsilon_n (-z^{n+1}\partial_z)\phi(z,\bar{z})+\bar{\epsilon}_n(-\bar{z}^{n+1}\partial_{\bar{z}})\phi(z,\bar{z})\,.
\end{split}
\end{equation}
Thus, we may define for each $n\in \mathbb{Z}$ the corresponding generators:
\begin{equation}
    \ell_n = -z^{n+1}\partial_z \, \quad \text{and} \quad \bar{\ell}_n=-\bar{z}^{n+1}\partial_{\bar{z}}\,. 
\end{equation}
We note that we obtain an infinite number of generators, which is to be expected given that the space of holomorphic and antiholomorphic functions is infinite dimensional. This is a very distinctive feature of the (local) conformal algebra in two dimensions. Furthermore, these generators satisfy the commutation relations of the Witt algebra:
\begin{equation}
    [\ell_m,\ell_n]=(m-n)\ell_{m+n}\,,\quad [\bar{\ell}_m,\bar{\ell}_n]=(m-n)\bar{\ell}_{m+n}\,,\quad [\ell_m,\bar{\ell}_n]=0\,.
\end{equation}
To make contact with the global conformal algebra defined in the previous section, we focus on the holomorphic generators $\{\ell_n\}$ of (one of the copies) of the Witt algebra. We note that there is an ambiguity in the definition at $z=0$, which motivates the introduction of the Riemann sphere $S^2\cong \mathbb{C}\cup \{\infty\}$, the conformal compactification of $\mathbb{R}^2\cong \mathbb{C}$. Nevertheless, even on the Riemann sphere, we have that 
\begin{equation}
    \ell_n = -z^{n+1}\partial_z \quad \text{is non-singular at $z=0$ for $n\geq -1$}\,.
\end{equation}
Similarly, for $z=\infty \in S^2$ we may perform a change of variables $z=1/w$ and study the limit $w \to 0$. We observe that 

\begin{equation}
    \ell_n = -\left(\frac{1}{w}\right)^{n-1}\partial_w \quad \text{is non-singular at $w=0$ for $n\leq +1$}\,.
\end{equation}
Hence, the only operators that are defined everywhere on the Riemann sphere are precisely $\{\ell_{-1},\ell_0,\ell_{+1}\}$ which satisfy an $\frak{sl}(2,\mathbb{R})$ algebra as expected. 

Therefore, we find that the local conformal algebra can be expressed as two copies of an infinite dimensional Witt algebra, such that each copy contains an $\frak{sl}(2,\mathbb{R})$ subalgebra corresponding to each of the $\frak{sl}(2,\mathbb{R})$ algebras contained in the global conformal Lie algebra. 

%the transformation, $x^\mu \mapsto y^\mu(x)$ the metric tensor transforms as:
%\begin{equation}
%\label{ec:metrictransf}
%    g^{\mu \nu} \to \left(\frac{\partial y^\mu}{\partial x^\alpha}\right)\left(\frac{\partial y^\nu}{\partial x^\beta}\right)g^{\alpha \beta} \,.
%\end{equation}
%The conformal condition $g'^{\mu \nu}(x)=\lambda(x)g^{\mu \nu}(x)$ implies two set of equations for the coordinates given by:
%\begin{equation}
%    \begin{array}{c}
 %    \displaystyle \left(\frac{\partial y^0}{\partial x^0}\right)^2+\left(\frac{\partial y^0}{\partial x^1}\right)^2=\left(\frac{\partial y^1}{\partial x^0}\right)^2+\left(\frac{\partial y^1}{\partial x^1}\right)^2  \\
  %   \\
  %  \displaystyle \left(\frac{\partial y^0}{\partial x^0}\right)\left(\frac{\partial y^1}{\partial x^0}\right)=\left(\frac{\partial y^0}{\partial x^1}\right)\left(\frac{\partial y^1}{\partial x^1}\right)
%\end{array}
%\end{equation}
%These conditions are equivalent to:

%\begin{equation}
%\label{ec:holocauchy}
%\frac{\partial y^{1}}{\partial x^{0}}=\frac{\partial y^{0}}{\partial x^{1}} \quad \text { and } \quad \frac{\partial y^{0}}{\partial x^{0}}=-\frac{\partial y^{1}}{\partial x^{1}}\,,
%\end{equation}
%or to
%\begin{equation}
%\label{ec:antiholocauchy}
%\frac{\partial y^{1}}{\partial x^{0}}=-\frac{\partial y^{0}}{\partial x^{1}} \quad \text { and } \quad \frac{\partial y^{0}}{\partial x^{0}}=\frac{\partial y^{1}}{\partial x^{1}} \,.
%\end{equation}
%We observe that equations \eqref{ec:holocauchy} and \eqref{ec:antiholocauchy} are the Cauchy Riemmann equations for holomorphic and antiholomorphic functions respectively. This motivates the definition of the complex variables and derivatives: 
%\begin{equation}
%    \begin{array}{c}
%z=x^{0}+i x^{1}\,, \quad \bar{z}=x^{0}-i x^{1}\,, \\
% \\
%\partial_{z}=\frac{1}{2}\left(\partial_{0}-i \partial_{1}\right) \,, \quad \partial_{\bar{z}}=\frac{1}{2}\left(\partial_{0}+i \partial_{1}\right)\,, \\
%\end{array}
%\end{equation}
%in terms of which the holomorphic and antiholomorphic Cauchy Riemann conditions may be expressed as:
%\begin{equation}
 %   \partial_{\bar{z}}y(z,\bar{z})=0\,, \quad \partial_{z}y(z,\bar{z})=0\,.
%\end{equation}
%This implies that any holomorphic or anti holomorphic transformation of the complex coordinates:
%\begin{equation}
%    z \to w(z) \quad \text{or}\quad \bar{z}\to \bar{w}(\bar{z})
%\end{equation}
%will result in a conformal transformation. It is \textbf{essential} to mention at this point, that the transformations considered herein are only defined \textit{locally}. We can infer this by looking at equation \eqref{ec:metrictransf} which is valid for local coordinate charts. Let us proceed by considering an infinitesimal conformal transformation:

\subsection{Conformal Field Theories in Two Dimensions}

Having discussed the local and global properties of conformal transformations of coordinates, we now focus in two dimensional field theories that are invariant under conformal transformations. In general, we know that symmetries of the classical action have associated conserved Noether currents. At the quantum level, these currents are slightly modified into the so known \textit{Ward Identities}. In this section we will look at the Ward identities associated to conformal symmetry transformations, paying close attention to the \textit{stress energy tensor}, which will play a fundamental role in this whole story. 

\subsubsection{The Stress Energy Tensor}

In any QFT, we can define the stress energy tensor $T^{\mu \nu}$ to be the Noether conserved current associated to space-time translations. In conformal field theories, the stress tensor has an additional very important property: it is traceless. Thus, we have
\begin{equation}
    \partial_\mu T^{\mu \nu}=0\,,\quad T^{\mu}{}_\mu = 0\,.
\end{equation}
In two dimensions, we may express these conditions using  complex coordinates. Traceleness then translates into $T_{z\bar{z}}=T_{\bar{z}z}=0$ while conservation implies $\partial_{\bar{z}} T_{zz}=0$ and $\partial_z T_{\bar{z}\bar{z}}=0$. This motivates the definition of the holomorphic and anti-holomorphic functions given by the non vanishing components of the stress tensor
\begin{equation}
T(z):=T_{zz} \quad \text{and} \quad \bar{T}(\bar{z}):= T_{\bar{z}\bar{z}}\,.
\end{equation} 
Let us now consider a general infintesimal conformal transformation of the holomorphic coordinate $z \to z+\epsilon(z)$, with $\epsilon$ an analytic function and $\bar{z}$ unchanged. Then the conserved current associated to this transformation is given by (c.f. \cite{tong})
\begin{equation}
\label{ec:jconserva1}
    J^z=0 \quad J^{\bar{z}}=T(z)\epsilon(z)\,.
\end{equation}
Similarly, for a conformal transformation in the $\bar{z}$ coordinate, we get the conserved current:
\begin{equation}
\label{ec:jconserva2}
    \bar{J}^{\bar{z}}=0 \quad \bar{J}^{z}=\bar{T}(\bar{z})\bar{\epsilon}(\bar{z})\,.
\end{equation}
Notably, we observe the appearance of the holomorphic and antiholomorphic components of the stress tensor in the expression for the conserved current of a general conformal transformation. 

\subsubsection{The Conformal Ward Identities}

Having established the form of the classical conserved currents related to general conformal transformations, we now turn to the quantum theory. As we mentioned before, the quantum version of Noether's theorem is encapsulated in the Ward Identities. Generally speaking, these tell us how do correlation functions of fields transform under a symmetry transformation of the action. If we restrict ourselves to consider conformal transformations, then under the usual transformation of the coordinates, $z\to z+\epsilon(z)$ and $\bar{z}\to \bar{z}+\bar{\epsilon}(z)$, the transformation of the correlation function of a product of arbitrary fields $ \phi_1(z_1,\bar{z}_1),\dots,\phi_n (z_n,\bar{z}_n)$ is given by (c.f chapter 5 of \cite{Francesco}):
\begin{equation}
\label{ec:wardidentity}
    \delta_{\epsilon \bar{\epsilon}}\langle X\rangle= -\frac{1}{2\pi i}\oint_C dz \epsilon(z) \langle  T(z) X \rangle + \frac{1}{2\pi i}\oint_C d\bar{z} \bar{\epsilon}(z) \langle  \bar{T}(\bar{z}) X \rangle\,,
\end{equation}
where we wrote $X=\phi_1(z_1,\bar{z}_1)\cdot \dots \cdot \phi_n (z_n,\bar{z}_n)$ and where the counterclockwise contour $C$ needs only to include the points were the fields are evaluated. As expected, we note the appearance of the non vanishing components of the classically conserved current $J^\bar{z}$ and $\bar{J}^z$ defined in equations \eqref{ec:jconserva1} and \eqref{ec:jconserva2} respectively, in each of the integrals.


\subsubsection{The Operator Product Expansion}
To gain some deeper insight on the expression of the conformal Ward identities given in equation \eqref{ec:wardidentity}, we introduce the operator product expansion (OPE). It is typical for correlation functions to have singularities when two or more fields coincide: This reflects the infinite fluctuations of a quantum field taken at a precise position. The OPE is the representation of a product of operators evaluated at $(z,\bar{z})$ and $(w,\bar{w})$ respectively, by a sum of single operators which are well defined as $(z,\bar{z})\to (w,\bar{w})$, multiplied by a function of $(z-w,\bar{z}-\bar{w})$ possibly divergent as $(z,\bar{z})\to (w,\bar{w})$. Concretely, let us denote by $\mathcal{O}_i$ the set of all operators in a given CFT. Then the OPE is:
\begin{equation}
    \langle\mathcal{O}_i(z,\bar{z})\mathcal{O}_j(w,\bar{w})\rangle=\sum_{k}C^{k}_{ij}(z-w,\bar{z}-\bar{w})\mathcal{O}_k(w,\bar
    {w})\,.
\end{equation}
The $c$-valued functions $C_{ij}^k$ which on ground of translational invariance depends on $(z-w,\bar{z}-\bar{w})$ contains all of the possible singularities arising in the product in the $(z,\bar{z})\to (w,\bar{w})$ limit. Given that the conformal Ward identities are expressed in terms of a contour integral, we will usually be interested \textit{only} in the singular behaviour of the OPE. As a matter of fact, we can classify fields with respect to their conformal transformation properties by looking at the OPE with the stress tensor. We say that an operator $\mathcal{O}(z,\bar{z})$ is a \textit{primary field} with weight $(h,\bar{h})$ if it has the following OPE with the stress tensor
\begin{equation}
\begin{split}
&\displaystyle T(z) \mathcal{O}(w, \bar{w})=h \frac{\mathcal{O}(w, \bar{w})}{(z-w)^{2}}+\frac{\partial \mathcal{O}(w, \bar{w})}{z-w}+\text { non-singular } \\
&\displaystyle \bar{T}(\bar{z}) \mathcal{O}(w, \bar{w})=\bar{h} \frac{\mathcal{O}(w, \bar{w})}{(\bar{z}-\bar{w})^{2}}+\frac{\bar{\partial} \mathcal{O}(w, \bar{w})}{\bar{z}-\bar{w}}+\text { non-singular }\,.
\end{split}
\end{equation}
Primary fields will play a key role when studying the representations of the conformal algebra in the next section. Notably, the stress energy tensor is not a primary field, which can be seen by computing the $TT$ self OPE. This can be shown to have the general expression:
\begin{equation}
    T(z)T(w)\sim \frac{c/2}{(z-w)^4}+\frac{2T(w)}{(z-w)^2}+\frac{\partial T(w)}{(z-w)}\,,
\end{equation}
where the $\sim$ symbol represents an equality modulo regular terms. We note the appearance of the $(z-w)^{-4}$ singular term which implies that $T(z)$ is not a primary field. The number $c$ is called the central charge of the theory and we will see its appearance throughout the whole text. 

\subsubsection{The Virasoro Algebra}

Within radial quantization, the OPE becomes a very strong computational tool. 

We have seen that the stress tensor is intimately related to the transformation properties of fields. Given the form of the Noether currents defined in equations \eqref{ec:jconserva1} and \eqref{ec:jconserva2}, we may define the conformal charge 
\begin{equation}
\label{ec:conformalcharge}
    Q_\epsilon = \frac{1}{2\pi i}\oint_C dz \epsilon(z)T(z)\,.
\end{equation}
We may further perform a Laurent expansion of the stress tensor 
\begin{align}
    T(z)&=\sum_{n\in \mathbb{Z}}z^{-n-2}L_n \quad \text{with} \quad L_n=\frac{1}{2\pi i}\oint_C dz z^{n+1}T(z)\,,\\
    \bar{T}(\bar{z})&=\sum_{n\in \mathbb{Z}}\bar{z}^{-n-2}\bar{L}_n \quad \text{with} \quad \bar{L}_n=\frac{1}{2\pi i}\oint_C dz \bar{z}^{n+1}\bar{T}(\bar{z})\,,
\end{align}
such that the charge reads, 
\begin{equation}
    Q_\epsilon =  \sum_{n\in \mathbb{Z}}\epsilon_n L_n\,, \quad Q_{\bar{\epsilon}}=\sum_{n\in \mathbb{Z}}\bar{\epsilon}_n \bar{L}_n
\end{equation}
where we have used the mode expansions for $\epsilon$ and $\bar{\epsilon}$ given in equation \eqref{ec:epsilonexpansion}.
Thus, the mode operators $L_n$ and $\bar{L}_n$ of the energy momentum tensor are precisely the generators of local conformal transformations in the Hilbert space, in the same way than the Witt generators $\ell_n$ and $\bar{\ell}_n$ are the generators of conformal transformations in the space of functions. There is however, a very subtle but important difference between these generators. If we compute the commutation relations between the modes of the energy momentum tensor we find:
\begin{subequations}
\begin{align}
    [L_n,L_m]&=(n-m)L_{n+m}+\frac{c}{12}n(n^2-1)\delta_{n+m,0}\\
    [L_n,\bar{L}_m]&=0\\
    [\bar{L}_n,\bar{L}_m]&=(n-m)\bar{L}_{n+m}+\frac{c}{12}n(n^2-1)\delta_{n+m,0}
\end{align}
\end{subequations}
which is the \textit{Virasoro} algebra. 

\subsection{Chiral Algebras}

The holomophic and an anti-holomorphic components of the stress tensor are examples of chiral and anti chiral operators respectively. In general, a chiral operator is a local operator $\mathcal{O}(z,\bar{z})$ that satisfies a meromorphicity condition of the form:
\begin{equation}
\label{ec:merocondition}
    \partial_{\bar{z}}\mathcal{O}(z,\bar{z})=0 \quad \Longrightarrow \quad \mathcal{O}(z,\bar{z}):=\mathcal{O}(z)
\end{equation}
Any operator satisfying such meromorphicity condition will give rise to the existence of an infinite number of conserved charges, obtained by integrating the operator against an arbitrary monomial in $z$:
\begin{equation}
    \mathcal{O}_n = \oint \frac{dz}{2 \pi i} z^{n+h-1}\mathcal{O}(z)\,,
\end{equation}
where $h$ is the holomorphic conformal dimension of the operator. Notably, the OPE of two meromorphic operators contains only meromorphic operators,  



, giving rise to an infinite number of conserved charges related to the modes of the Laurent expansion. These strongly constrain the correlation functions of the theory via the Ward identities. However, generic operators in two dimensional CFT's will exhibit both holomorphic and anti-holomorphic dependence and thus, correlation functions only make sense once the holomorphic and anti-holomorphic behaviour is well understood. 



Chiral symmetry arises as a consequence of the existence of any local operator $\mathcal{O}(z,\bar{z})$ which obeys a meromorphicity condition:

 The operator product expansion of two meromorphic operators contains only meromorphic operators, and the singular terms determine the commutation relations among the associated charges, cf. [25deLiendo]. The algebra of these conserved charges is called a \textit{chiral algebra}.

In the previous section we observed that the energy momentum tensor splits into a holomorphic and antiholomorphic component, each of which satisfies a meromorphicity condition as in equation \eqref{ec:merocondition}. Furthermore, we saw that the modes of the mode expansion of either component satisfy the commutation relations of the Virasoro algebra. Thus, the modes of the energy stress tensor span a chiral algebra, which in this case, is the Virasoro algebra. 




\subsection{The Conformal Bootstrap}

We see that the complete information to specify a two dimensional conformal field theory is provided by the conformal weights $(h_i,\bar{h}_i)$ of the Virasoro
highest weight states, and the operator product coefficients $C_{ijk}$ between the
primary fields that create them. Everything else follows from the values of
these parameters, which themselves cannot be determined solely on the basis
of conformal symmetry. To determine the unspecified $C_{ijk}$ and the conformal weights, we consider the four point function
\begin{equation}
\left\langle\phi_{1}\left(z_{1}, \bar{z}_{1}\right) \phi_{2}\left(z_{2}, \bar{z}_{2}\right) \phi_{3}\left(z_{3}, \bar{z}_{3}\right) \phi_{4}\left(z_{4}, \bar{z}_{4}\right)\right\rangle\,.
\end{equation}
Since the order in which fields appear within the correlation function doesn't matter, we have different ways of computing the double OPE, which correspond to the different choices of the fields that intervene in the single OPE. For example, we can compute the four point function as the double OPE
\begin{equation}
\label{ec:fourpoint1}
\left\langle\left[\phi_{1}\left(z_{1}, \bar{z}_{1}\right) \phi_{2}\left(z_{2}, \bar{z}_{2}\right)\right]\left[ \phi_{3}\left(z_{3}, \bar{z}_{3}\right) \phi_{4}\left(z_{4}, \bar{z}_{4}\right)\right]\right\rangle
\end{equation}
where the square brackets indicate that the OPE is taken between the fields inside. But we could as well, consider:
\begin{equation}
\label{ec:fourpoint2}
\left\langle\left[\phi_{1}\left(z_{1}, \bar{z}_{1}\right)\phi_{3}\left(z_{3}, \bar{z}_{3}\right) \right]\left[\phi_{2}\left(z_{2}, \bar{z}_{2}\right)  \phi_{4}\left(z_{4}, \bar{z}_{4}\right)\right]\right\rangle\,.
\end{equation}
If we want our operator algebra to be associative, then (assuming the fields are not Grassman valued) equations \eqref{ec:fourpoint1} and \eqref{ec:fourpoint2} should coincide. This requirement is a consistency condition, known as the crossing symmetry of the four point function. This implies an infinite number of equations that the $C_{ijk}$ must satisfy. 

MIRAR PAGINA 201 DEL FRANCESCO


